Exposing Fake Images with Forensic Similarity Graphs

We propose new image forgery detection and localization algorithms by recasting these problems as graph-based community detection problems. To do this, we introduce a novel abstract, graph-based representation of an image, which we call the Forensic Similarity Graph, that captures key forensic relationships among regions in the image. In this representation, small image patches are represented by graph vertices with edges assigned according to the forensic similarity between patches. Localized tampering introduces unique structure into this graph, which aligns with a concept called ``community structure'' in graph-theory literature. In the Forensic Similarity Graph, communities correspond to the tampered and unaltered regions in the image. As a result, forgery detection is performed by identifying whether multiple communities exist, and forgery localization is performed by partitioning these communities. We present two community detection techniques, adapted from literature, to detect and localize image forgeries. We experimentally show that our proposed community detection methods outperform existing state-of-the-art forgery detection and localization methods, which do not capture such community structure.

==> figs/vtl/vtl_fig1.tex <==
\begin{figure}
\null\hfill
\begin{subfigure}[t]{0.7\linewidth}
\centering
\includegraphics[width=\linewidth]{figs/vtl/vtl_roc_256cnn_256block.pdf}
\caption{ROC, $256 \times 256$ Forgery Block Size}
\end{subfigure}
\hfill\null
%\begin{subfigure}[t]{0.32\linewidth}
%\centering
%\includegraphics[width=\linewidth]{figs/vtl/vtl_roc_mean_Average_Precision_cnn256.pdf}
%\caption{mAP by Forgery Block Size}
%\end{subfigure}
%\hfill

\null\hfill
\begin{subfigure}[t]{0.7\linewidth}
\centering
\includegraphics[width=\linewidth]{figs/vtl/vtl_roc_PD_at_PFA05_cnn256.pdf}
\caption{$P_D$ at $P_{FA}=0.05$ by Forgery Block Size}
\end{subfigure}
\hfill\null
\caption{Synthetic Forgery Result}
\label{fig:vtl_result_1}
\end{figure}

==> figs/vtl/vtl_fig2.tex <==
\begin{figure}
\null\hfill
\begin{subfigure}[t]{0.85\linewidth}
\centering
\includegraphics[width=\linewidth]{figs/vtl/vtl_auc_vs_forgery_size_Spectral_Gap.pdf}
\caption{AUC by Forgery Block Size}
\end{subfigure}
\hfill\null

\null\hfill
\begin{subfigure}[t]{0.85\linewidth}
\centering
\includegraphics[width=\linewidth]{figs/vtl/vtl_auc_vs_forgery_size_Spectral_Gap_relative.pdf}
\caption{AUC by Relative Size of Forgery Block}
\end{subfigure}
\hfill\null
\caption{Area Under the Curve of Spectral Gap method on synthetic forgeries for two forensic patch sizes.}
\label{fig:vtl_result_2}
\end{figure}

==> sections/approach.tex <==
\section{Forensic Graph Representation}
\label{sec:approach}
In this paper, we propose an approach to detect and local image forgeries. To do this we first convert the image into a graph representation that has image patches as vertices with fully connected edges, and where each edge is assigned weight according to the forensic similarity between two vertices. In forged images, the tampered regions will form ``communities'' that can be detected, in the case of forgery detection, and partitioned, in the case of forgery localization. 

Generally, the proposed procedure is as follows:
\begin{enumerate}
\item Convert the image into it's forensic graph representation
\item Forgery detection: detect the presence of more than one community in the forensic graph\\ 
or \\
Forgery localization:  partition the graph into disjoint communities
\end{enumerate}

In this section, we describe how the forensic graph is constructed from an image, and show how clusters, or ``communities,'' are present in the forensic similarity graph in the case where the image has undergone forgery. In the following section, we introduce describe how community detection techniques can be applied to this graph to both detect image forgeries and localize the tampered regions.

%In forged images where tampering is not applied uniformly across the image, this representation forms distinct highly in-connected communities that are relatively disconnected across communities.

%
%describe how we grid/patch image
%describe how we calculate the forensic similarity
%
To construct the forensic graph of an image, we first sample $N$ patches from the image $\left\lbrace X_1, X_2, \ldots, X_N \right\rbrace$. In this paper we use square patches that are regularly spaced and overlapped, typically we use a patch size of $128\times128$ and 50\% overlap. However, we note the proposed technique is general to irregulary shaped patches and arbitrary locations. 
We then construct a graph $G=(V,E)$ with vertex set $V = \left\lbrace v_1, \ldots, v_n \right\rbrace$ where $v_i$ represents the $i^{th}$ sampled patch in an image. The graph has edges $E$ which connect the vertices. In this work edges are fully connected with weight $W_{i,j}$ equal to the forensic similarity between $v_i$ and $v_j$. That is, the graph has edge weights,
%
\begin{equation}
W_{i,j} = \fsim{X_i}{X_j},
\end{equation}
%
where $W_{i,j}$ is the edge weight between vertex $i$ and vertex $j$, and $\fsim{X_i}{X_j}$ is the forensic similarity between image patch $X_i$ and image patch $X_j$. 

Here, we use forensic similarity $S(\cdot,\cdot)$ as defined in~\cite{mayer2019similarity}. Forensic similarity is a technique that maps two image patches, $X_1$ and $X_2$, to a score $\in [0,1]$. A low score near $0$ indicates that the two image patches have different forensic traces, and a high score near $1$ indicates that they have the same forensic traces. The research in~\cite{mayer2019similarity} shows that, depending on training setup, these forensic traces can be indicative of source camera model and/or processing history. 
As a result, edge weight $W_{i,j}$ is based on the similarity of the source and/or processing history of patches $X_i$ and $X_j$. The edge weights create the edge weight matrix, which we refer to as the \textit{Forensic Similarity Matrix}. In some literature, this edge weight matrix is referred to as a weighted affinity matrix, or weighted adjacency matrix.\looseness=-1

Structures in this forensic graph are used to identify and localize image forgeries. In forged images (e.g. a spliced image), it is expected that an edge between a patch in the tampered region and a patch in the unaltered image region will have low weight. Edges between patches from the unaltered part of the image have high weight, since all unaltered patches have undergone the same processing history. Additionally, edges between patches in a tampered region have high weight, provided that the entirety of the tampered region has undergone the same tampering process (e.g. brush tool, resizing, etc) and were sourced from the same camera model. Alternatively in unaltered images, where every patch was captured by the same camera model and has the same processing history, all edges in the graph are expected to have high weight.

These high-weight edges within the unaltered region and tampered region(s), and low-weight edges across the unaltered region and tampered region(s) form what is called "community structure" ~\cite{}. This is akin to a graph of a social network where vertices represent people with edges according to their connections (e.g. follows, likes, etc.). People within a community tend have high connections within their community, and low connections outside of the community. There exists a breadth of research and techniques to analyze community structure in graphs, including techniques to identify the existence of these communities and to partition the communties~\cite{fortunato2010community}. By leveraging this research and applying these techniques to an image's Forensic Graph, we can detect the presence of forgery in an image and identify the tampered regions.

We assume that tampering has occurred non-uniformly across this image. This includes, for example, a splicing forgery or a localized application of a brush tool. This does not include global operation such as gamma correction or global resizing. While important, we consider the detection of global manipulations to be a separate problem. As a result of localize tampering, the graph of the forged image contains clusters of patches, referred to as  communities, that have high-weight edges within their community, and low-weight edges to vertices outside their community. These communities correspond to each tampered and unaltered regions. An example of this can be seen in Fig.~\ref{fig:simgraph_example}(d), which shows two communities in the forged image: one community in green corresponding to the tampered patches, and one in red corresponding to the unaltered patches. In the case where no localized tampering has occurred, only one such community exists.

%A forged image may have multiple tampered regions, which, in this framework, are delineated by differences in forensic traces. Edge weights between two tampered regions are of low weight.

%These weights take high values when the two image patches have a similar forensic properties. These forensic properties include attributes such as source camera model and/or processing history~\cite{mayer2019similarity}. 

%To construct this graph from an image, we grid the image into overlapping square patches and assign a vertex in the graph to represent an individual patch. In this paper, we use patch sizes of $128 \times 128$ or $256 \times 256$ with 50\% overlap in each dimension. We refer to this size as \textit{forensic patch size}. However, this method is trivially extendable to other patch sizes and overlap amounts. To determine edge weights, we then calculate the forensic similarity between each pair of patches. With the vertices (image patches) and edges weights (forensic similarity) determined, the graph is fully specified.

\subsubsection{Example} As an example, in Fig.~\ref{fig:simgraph_example} we show (b) a tampered image, and (a) the corresponding original image. In this tampered image, the person's shirt has been edited using a brush tool to remove the appearance of rain drops on their shirt. The tampered image is gridded into $256\times256$ patches, with 50\% overlap. An index is assigned to each vertex and are shown in Fig.~\ref{fig:simgraph_example}(b) at their corresponding patch locations. 

In this example, from the edge weight matrix shown in Fig.~\ref{fig:simgraph_example}(c), it can be seen that the vertices corresponding to the edited shirt patches, indices = $\lbrace 14, 15, 16, 21, 22, 23, 28, 29 \rbrace$, have low similarity to the rest of the image patches, and high similarity to other edited shirt patches. Similarly, the non-edited patches have low similarity to the edited patches, and high similarity to other non-edited patches. This suggests that in this tampered image example, there are two forensic "communities". Interestingly, patches that appear on the boundary of the tampered/unaltered boundary, indices = $\lbrace 17, 24, 25, 30, 35, 36\rbrace$, have high similarity to both the edited and non-edited patches.

In Fig.~\ref{fig:simgraph_example}(d), the vertex-edge representation of this graph is shown. For visualization purposes, we only draw edges between vertices that have forensic similarity $>0.90$. This visual representation clearly highlights that two communities exist, one associated with the tampered region, and one associated with the non-tampered region. Vertex colors are assigned according to the partitioning determined by the a ``modularity optimization'' method~\cite{newman2004finding}, with edges between communities grayed out. The graph is arranged according to the Kamada-Kawai force directed algorithm~\cite{kamada1989algorithm}. Layout and partitioning were performed using the \textit{igraph} software package~\cite{igraph}.



==> sections/background_rework.tex <==
\section{Background and Related Work}
\label{sec:related}
\subsection{Image Forgery Detection and Localization}
Multimedia forensics techniques explicitly draw the distinction between forgery detection and forgery localization. Forgery \textit{detection} methods are those that determine if an image has been tampered or is alternatively unaltered. Forgery \textit{localization} methods are those that, given a forged image, determine which regions of an image have been tampered. While these are distinctly different problems, the underlying mechanisms for analysis are similar and, as a result, are often studied in conjunction. In this paper, we propose techniques for both forgery detection and forgery localization.

Recently, researchers have leveraged advances in deep learning to perform both forgery detection and forgery localization with high accuracy. In early work by Bondi et al. a convolutional neural network (CNN) was used to generate deep-feature representations of an image's source camera-model, and then detected and localized image forgeries via an iterative k-means clustering approach~\cite{bondi2017cvprw}. Subsequently, our work in~\cite{mayer2018similarity} showed that similarity of camera-model related forensic traces can be directly measured using a CNN-based siamese network, which can be used to localize image forgeries. This idea was further refined by our research in~\cite{mayer2019similarity}, where we proposed a more formal definition of Forensic Similarity, which is the quantifiable measure of similarity of forensic traces related to the source and/or processing between two images patches, and refined the siamese network technique.

Deep learning forensics research by Cozzolino et al.~\cite{cozzolino2018noiseprint,cozzolino2018camera} proposed a CNN that transforms an image to highlight artifacts associated with camera-specific traces. Inconsistencies in the resulting fingerprint map were then used to identify forged regions. Huh et al. developed a deep-learning technique to create a ``consistency map'' for forged images~\cite{huh2018forensics}. In this consistency map approach, regions of the image are highlighted which contain predictions of EXIF-based metadata that are inconsistent with the majority of the image. Huh et al. showed that taking spatial average of the consistency map and comparing to a threshold can be used to perform forgery detection.

The work in this paper directly builds from our prior research on Forensic Similarity in~\cite{mayer2019similarity}. In our prior work, we showed that tampered regions of an image can be localized by selecting reference patch, and highlighting the patches in the image that contain different forensic traces. Provided a patch in the unaltered region of the image was selected, the tampered regions would are highlighted. Furthermore, we showed state-of-the-art forgery detection accuracy by computing the forensic similarity values between all patches, computing the mean of these values, and comparing that mean to a threshold. In unaltered images, this value would be high indicating all patches were forensically similar. Alternatively in tampered images, this value would be low indicating some patches were forensically dissimilar.

However, there are drawbacks to the existing forgery detection and localization approaches using Forensic Similarity. First, the forgery localization approach required a selection of a reference patch in the image. This is problematic since the investigator may not have knowledge of which regions of the image are unaltered, and the poor selection of a patch may lead to erroneous results. Second, the forgery detection approach, which utilized the mean forensic similarity value of the image, does not adequately consider the complex forensic relationships that occur in a tampered image. For example, a large tampered region will be self-similar within the region, but dissimilar to the unaltered part of the image. This type of relationship is lost by averaging all similarity values. Furthermore, by utilizing the mean similarity value, the detection statistic becomes inherently tied to the size of the forged region. However, it is important to be able to detect forgeries. This problem also occurs in the forgery detection approach in~\cite{huh2018forensics}, which utilizes the spatial average of the EXIF consistency map to detect forgeries.

In this paper, we propose techniques that address these drawbacks. To do this, we build a graph-based representation of the image, called the Forensic Graph Representation. This representation uses a graph to capture the forensic relationships among all patches of the image. In images that images with localized tampering, the tampered regions form communities in this graph. As a result, the graph can be analyzed for the existence of multiple communities, indicating tampering, and those communities can be partitioned to localize the tampered regions. By taking this approach, the proposed methods leverage the complex relationships captured by the graph representation to more accurately detect forgeries and localize tampered regions without, addressing the drawbacks of the existing Forensic Similarity approaches in~\cite{mayer2018similarity} and~\cite{mayer2019similarity}. 

\subsection{Community Detection in Graphs}


A graph, $G$, is an abstract representation that captures the relationships among a set of objects. The graph $G=(V,E)$ is defined by a set of vertices (objects) $V$
and edges $E$ which connect each unique pairing of vertices. Edges may be weighted or binary. In this work, we propose a graph-based representation of images. In Sec.~\ref{sec:approach}, we will show how to detect and localize forgeries by partitioning structures, called \textit{communities}, in this graph representation.

To identify and partition communities in graphs, researchers have developed a number of techniques called ``community detection'' algorithms~\cite{fortunato2010community}. In this paper, we will directly build from two popular and successful techniques, namely Modularity Optimization~\cite{girvan2002community} and Spectral Clustering~\cite{von2007tutorial}. Modularity is a quality index of how well a graph is partitioned into communities~\cite{fortunato2010community}. Modularity Optmization is a family of techniques that find high quality partitions of graphs by optimizing for Modularity. A second technique we build off of is Spectral Clustering~\cite{von2007tutorial}. Spectral Clustering defines a matrix, called the graph Laplacian, whose eigenvector spectrum has unique properties. In particular, the eigenvalues of the graph Laplacian contains clues about the number of communities that exist, and the component values of the eigenvectors can be used to accurately partition the graph in communities~\cite{von2007tutorial}.

Spectral clustering is a technique for partitioning graphs into clusters~\cite{fortunato2010community,von2007tutorial,chung1996spectral}, which leverages properties of the graph Laplacian matrix to determine community structures.

The graph Laplacian matrix, $L$, is defined as
\begin{equation}
L = D-W,
\label{eq:graph_laplacian}
\end{equation}
where $W$ is the edge weight matrix with elements, %\mbox{$W_{i,j} = S(X_i,X_j)$} equal to the forensic similarity between image patches $X_i$ and $X_j$
and $D$ is the degree matrix with values
\begin{equation}
D_{ii} = \sum_j W_{ij}
\end{equation} 
on the diagonal, and zeroes off-diagonal. 
Additionally, the \textit{normalized} graph Laplacian 
\begin{equation}
L_{norm} = D^{-\frac{1}{2}}LD^{-\frac{1}{2}},
\end{equation}
is a regularized version of the matrix.

The graph Laplacian has a number of special properties. In particular, it has spectrum of non-negative real valued eigenvalues $0= \lambda_1 \leq \lambda_2 \leq \ldots \leq \lambda_n$. These eigenvalues a have property such that the multiplicity of $\lambda=0$ is equal to the number of disconnected communities in the graph. Furthermore, the eigenspace of $0$ is spanned by the indicator vectors $\mathbbm{1}_{A_1},...,\mathbbm{1}_{A_k}$ of those k communities, where $A_i$ is the vertex membership of the $i^{th}$ community. For the normalized graph Laplacian, it this eigenspace spanned by $D^{\frac{1}{2}}\mathbbm{1}_{A_1}$~\cite{von2007tutorial,chung1996spectral}. We use these properties for detecting forgeries and localizing the forged regions, described further in Sec.~\ref{sec:approach}.


Modularity, $Q$, is an index for the quality of how well a graph has been partitioned into communities~\cite{fortunato2010community}, defined as:
%
\begin{equation}
Q = \frac{1}{4m}\sum_{i,j}\left(W_{ij}-\frac{d_id_j}{2m}\right)\mathbbm{1}(c_i = c_j)
\end{equation}
%
where $m$ is the sum of edges in the graph, $W$ is the edge weight matrix, $d_i$ is the weighted degree of node $i$, and the indicator function $\mathbbm{1}(c_i = c_j)$ is 1 when both node $i$ and $j$ are assigned to be members of the the same community. 
%
The term $\frac{d_id_j}{2m}$ is interpreted as the expected weight of a randomly occurring connection between vertices $i$ and $j$. Intuitively, if two vertices in the same community have a low connection expectation, but have a high weight between them, then modularity is increased.

Modularity Optimization is a family of techniques used to determine the underlying community memberships in a graph. These techniques operate by assign vertices to communities such that modularity is maximized, %We can find the community assignments that maximize modularity for the graph using an optimization method. 
\begin{equation}
Q_{opt} = \max_{\{c_1, \ldots, c_n \}} \frac{1}{4m}\sum_{i,j}\left(W_{ij}-\frac{d_id_j}{2m}\right)\mathbbm{1}(c_i = c_j).
\end{equation}
Higher values of modularity indicate that community structure exists, and that a good partitioning has been found~\cite{fortunato2010community,newman2004finding,girvan2002community}. Modularity in the case of a single community is zero. 

To calculate $Q_{opt}$, in Sec.~\ref{sec:approach} we use a popular modularity optimization technique called the ``fast-greedy'' method, which agglomeratively forms communities by iteratively combining communities which yield the greatest modularity increase~\cite{newman2004fast,clauset2004finding}, and reports the largest modularity value found. While there are a number of variations of modularity optimization techniques, the fast-greedy method is a popular technique~\cite{fortunato2010community} and operates on a reasonable timescale on our forensic graphs. 




==> sections/community_detection_rework.tex <==
\section{Community Detection}
\label{sec:approach:ssec:detection}
%In this work, we explore a graph-based method for detecting whether a tampering has occurred in the image. These methods operate by identifying the presence of multiple communities in the image's forensic graph representation.
In the previous section, we introduced the Forensic Graph Representation of an image and provided intuition about how structures in this representation, called ``communities," indicate that the image has been locally tampered. In this section, we introduce techniques to detect and analyze this community structure in graphs in order to accurately detect forgeries and localize those tampered regions.

Forgery detection and forgery localization are two related, but very different problems in multimedia forensics, and are differentiated in literature~\cite{bondi2017cvprw,huh2018forensics}. Forgery detection techniques are used to indicate whether tampering has occurred in the image, and output a binary yes/no decision about the image. In this work, we propose community detection techniques that input a forensic graph and output a forgery detection decision,
\begin{align}
\text{Forgery Detection}(G) \rightarrow  & \left\lbrace \text{Image is Unaltered,} \right. \\ & ~ \left. \text{Image is Forged} \right\rbrace,
\end{align} 
We also propose community detection techniques that input a forensic graph, and output a tampering classification for each patch of the image, which is then used to segment the tampered regions of the image,
\begin{equation}
\text{Forgery Localization}(G) \rightarrow \left\lbrace c_1, c_2, \ldots, c_n \right\rbrace,
\end{equation}
where $c_i \in \left\lbrace 1, \ldots, k \right\rbrace$ is the community membership for the $i^{th}$ vertex in the graph, i.e. sampled image patch, and $n$ is the number of sampled image patches. We note that the nature of this type of localization analysis partitions the tampered region from the unaltered, but does not inherently identify which of the partitioned regions is the tampered one or unaltered one. This is why each vertex/patch is mapped into a community identifier $\left\lbrace 1, \ldots, k \right\rbrace$ as opposed to $\left\lbrace\text{Unaltered}, \text{Forged}\right\rbrace$. In this paper we focus on the case of $k=2$, since the experimental databases we evaluate on present only one tampered region, however the techniques we propose are general to any integer $k$. Recent work has highlighted the need for techniques that work on more than one tampered region~\cite{hosseini2019unsupervised}.

In the remainder of this section, we introduce two community detection techniques from literature, namely Spectral Clustering and Modularity Optimization, and adapt them to the problems of image forgery detection and localization. While there exists many different community structure analysis techniques, spectral clustering and and modularity optimization are two of the most popular and successful techniques~\cite{fortunato2010community}.

Additionally, we show how to convert the patch-based localization partitions, which result from the community detection methods, into a pixel-level segmentation of forged and unaltered regions. This is done so that the proposed localization methods can be effectively compared to other forgery localization techniques that operate at the pixel-level, such as those in~\cite{cozzolino2015splicebuster,bondi2017cvprw,huh2018forensics}.
%Before introducing these techniques, we first make explicit the two problems that we are addressing: 1) forgery detection and 2) forgery localization. 


%asdf


%As a result, by identifying the existence of more than one community, we identify the image as forged. There exists a rich body of literature on detecting community related structure in graphs~\cite{fortunato2010community}, which we leverage in this work.
%
%[Brief description of community detection measures]
%
%The first technique, which we refer to as the Spectral Gap, leverages spectral properties of the graph Laplacian matrix. The second technique, which is called Modularity Optimization, finds a partition of the graph that optimizes modularity, a measure of community structure. The resulting measures of these two techniques are then used as a measure for tampering detection. In our experimental results, we compare the efficacy of each approach, as well as compare to naive approaches that do not consider community structure and to prior art.
%


\subsection{Spectral Clustering}
In this method, we adapt a technique called Spectral Clustering to the forensic graph representation to detect forgeries and/or localize tampered regions.  %Go over background of spectral clustering in the background section 

%We note that this method does not indicate which regions or individual pixels are tampered, just that a tampering has occurred in the image. While related, this type of approach is importantly distinct from forgery localization, which classifies individual pixels as either being unaltered or forged. Since the underlying similarity measure is performed at the patch level, this technique does not immediately translate to pixel-based forgery localization.


\input{figs/forgery_detection_examples.tex}
\subsubsection{Forgery Detection}

Here we use the fact that the multiplicity of $\lambda=0$ is equal to the number of disconnected communities in the graph to decide whether an image has been forged. Typically, this multiplicity is used to determine the number of communities in graph by determining the number of consecutive eigenvalues less than a threshold, and is sometimes called the ``Eigengap" heuristic~\cite{von2007tutorial}. However, the problem of forgery detection is different in that we need to know only whether the image is forged or unaltered. In other words, we are concerned only if there exists a single community (unaltered) or, alternatively, more than one community (localized tampered).
%The graph Laplacian matrix has well studied properties~\cite{chung1996spectral}. In particular, it has spectrum of non-negative real valued eigenvalues $0= \lambda_1 \leq \lambda_2 \leq \ldots \leq \lambda_n$. These eigenvalues a have property such that the multiplicity of $\lambda=0$ is equal to the number of disconnected communities in the graph~\cite{von2007tutorial,chung1996spectral}.
%In this method, we calculate the spectrum $\lbrace \lambda_1 , \ldots , \lambda_n \rbrace$ of the graph Laplacian as described in Sec.~\ref{sec:background:ssec:community}. The spectrum has a property such that the multiplicity of $\lambda=0$ indicates the number of connected communities that exist. 
%This property is often used by a technique called the ``Eigen Gap" method, used to determine the number of clusters in dataset~\cite{}. 

To do this, in our approach we calculate the second smallest eigenvalue $\lambda_2$. If this value is low, it is indication that at least two communities exist, and potentially more. If it is high, then it is an indication only one community exists, and the image has not been altered. 
%
As a result, our forgery detection decision rule becomes
\begin{align}
\text{Spectral Gap}\left(G \right) =  \begin{cases}
\text{Unaltered}, & \lambda_2 \geq \tau\\
\text{Forged}, & \lambda_2 < \tau,
\end{cases}
\end{align}
where $G$ is the forensic graph representation of the image, $\lambda_2$ is second smallest eigenvalue of the graph Laplacian from Eq.~\eqref{eq:graph_laplacian}, and $\tau$ is the decision threshold determined empirically depending on the desired operating point.

Examples of the spectral gap are shown in Fig.~\ref{fig:detection_examples} for unaltered and forged images. In the two unaltered images(a) and (c) the spectral gap values of 318.42 and 235.56 are high, indicating that only one forensic community exists and no tampering has occurred. In the two spliced images (b) and (d) the spectral gap values of 76.75 and 4.28 are low, indicating that more than one forensic community exists and the tampering has occurred.

\subsubsection{Forgery Localization}
To perform localization, we use the fact that the eigenspace of $0$ of the graph Laplacian is spanned by the indicator vectors $\mathbbm{1}_{A_i}$ to partition the graph vertices into forged and unaltered regions. In this paper we consider the case of $k=2$, in order to partition the tampered versus unaltered regions. %We sign of each component the eigenvector $\mathbf{u}_2 \in \mathbb{R}^n$ of the second smallest eigenvalue to partition each vertex/image patch into separate communities
To do this, we first calculate the eigenvector $\mathbf{u}_2 \in \mathbb{R}^n$ associated with the eigenvector $\lambda_2$
\begin{equation}
\mathbf{L} \mathbf{u}_2 = \lambda_2 \mathbf{u}_2,
\end{equation}
where $\lambda_2$ is the second smallest eigenvalue of the graph Laplacian matrix.

Next, we use the sign of each component of $\mathbf{u}_2$ to assign each vertex into a community membership,
\begin{align}
\hat{c}_i =  \begin{cases}
1, & u_{i,2} \geq 0\\
2, & u_{i,2} < 0,
\end{cases}
\end{align}
where $\hat{c}_i$ is the predicted community membership of the $i^{\text{th}}$ graph vertex / image patch. This method approximates the (NP-Hard) Ratio cut algorithm for k=2. When using the normalized graph Laplacian, it approximates the Normalized Cut algorithm~\cite{von2007tutorial}.

An example of this algorithm is shown in Fig.~\ref{fig:sc_partition_example}, where we partition the image patches from the spliced image in Fig.~\ref{fig:detection_examples}(d) into two communities. In this figure, we show the histogram of values of $\mathbf{u}_2$. The components associated with patches in the tampered region are shown in blue, and are typically above 0. The components associated with patches in the unaltered regions are shown in orange, and are typically below 0. Ground truth was determined based on the central location of each image patch.

We note that this algorithm can be easily extended to consider $k>2$. This is done by considering the eigenvector values for each vertex as a point in space and performing k-means clustering~\cite{von2007tutorial}. 

\begin{figure}[t]
\centering
\includegraphics[width=0.66\linewidth]{figs/jt_veig_componentvalues.pdf}
\caption{Component values of $\mathbf{u}_2$ for the edited image in Fig.~\ref{fig:detection_examples}(d). In this example, components of $\mathbf{u}_2$ corresponding to the forged patches are greater than 0, and unaltered patches are less than 0.}
\label{fig:sc_partition_example}
\end{figure}

\subsection{Modularity Optimization}
Here, we apply a 2nd community detection technique for forgery detection and localization. In this method, we use a technique called Modularity Optimization to the Forensic Graph Representation to detect and localize forgeries. 

\subsubsection{Forgery Detection}
To detect whether the image has been locally tampered, we compare the optimized modularity value, $Q_{opt}$, found for the optimal partition to a threshold. If $Q_{opt}$ exceeds the threshold, it indicates that there is strong community structure and, as a result, indicates that one or more regions of the image has been tampered with. Our decision measure becomes 
%
\begin{align}
\text{Modularity Opt}\left(G \right) =  \begin{cases}
\text{Unaltered}, & Q_{opt} < \tau\\
\text{Forged}, & Q_{opt} \geq \tau,
\end{cases}
\end{align}
%
where $G$ is the forensic graph representation of the image, $Q_{opt}$ is the optimized modularity value found on $G$, and $\tau$ is the decision threshold, chosen empirically.

\subsubsection{Forgery Localization}

Here, we localize tampered regions by using the optimized community memberships, $\hat{c}$, to assign each patch into a community,
%
\begin{equation}
\{\hat{c}_1, \ldots, \hat{c}_n \} = \argmax_{\{c_1, \ldots, c_n \}} \frac{1}{4m}\sum_{i,j}\left(W_{ij}-\frac{d_id_j}{2m}\right)\mathbbm{1}(c_i = c_j)
\end{equation}
%
where $\hat{c}_i \in \lbrace 1, \ldots, k \rbrace$ is the optimized community membership of the $i^\text{th}$ vertex/image patch determined by the modularity optimization algorithm. As with the Spectral Clustering method, we use $k=2$ to segment the unaltered region from the forged region(s). Though we note that this method is trivially extendable to $k>2$.

As an example, the partitioning into the green and red coloring of Fig~\ref{fig:simgraph_example} was determined by the Modularity Optimization method, using an edge weighting threshold of $t=0.9$ and $k=2$.



==> sections/preamble.tex <==
\copyrightyear{2019} 
\acmYear{2019} 
\setcopyright{acmlicensed}
%\acmConference[IH\&MMSec '18]{6th ACM Workshop on Information Hiding and Multimedia Security}{June 20--22, 2018}{Innsbruck, Austria}
\acmBooktitle{IH\&MMSec '19}
\acmPrice{}
\acmDOI{}
\acmISBN{}

\author{Owen Mayer}
\affiliation{%
  \institution{Drexel University}
  %\department{Department of Electrical and Computer Engineering}
  \city{Philadelphia} 
  \state{PA}
  \country{USA}
}
\email{om82@drexel.edu}

\author{Luca Bondi}
\affiliation{%
  \institution{Politecnico di Milano}
  %\department{}
  \city{Milan} 
  \country{Italy}
}
\email{luca.bondi@polimi.it}

\author{Matthew C. Stamm}
\affiliation{%
  \institution{Drexel University}
  %\department{Department of Electrical and Computer Engineering}
  \city{Philadelphia} 
  \state{PA}
  \country{USA}
}
\email{MStamm@coe.drexel.edu}


% The default list of authors is too long for headers.
\renewcommand{\shortauthors}{O. Mayer et al.}

\settopmatter{printacmref=true, printccs=false, printfolios=true}



%
% The code below should be generated by the tool at
% http://dl.acm.org/ccs.cfm
% Please copy and paste the code instead of the example below.
%
% The code below should be generated by the tool at
% http://dl.acm.org/ccs.cfm
% Please copy and paste the code instead of the example below. 
%
\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10010147.10010371.10010382.10010383</concept_id>
<concept_desc>Computing methodologies~Image processing</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10002978.10002991.10002992</concept_id>
<concept_desc>Security and privacy~Authentication</concept_desc>
<concept_significance>500</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Security and privacy~Authentication}
\ccsdesc[500]{Computing methodologies~Image processing}


\keywords{Multimedia forensics, forgery detection, forensic similarity, community detection}

==> tables/localization.tex <==
\begin{table}
\center
\caption{MCC, per image threshold}
\vspace{-0.5em}
\begin{tabular}{l c c c}
\toprule
 & Columbia & Carvalho & Korus \\
 \midrule
Splice Buster~\cite{cozzolino2015splicebuster} & 0.68 & 0.56 & 0.34 \\
Bondi et al.~\cite{bondi2017cvprw} & 0.50 & 0.35 & 0.22 \\
%Huh et al. ``EXIF"~\cite{huh2018forensics}(reported) & 0.80 & 0.42 &  \\
Huh et al. EXIF~\cite{huh2018forensics} & \textbf{0.87} & 0.46 & 0.23 \\
\midrule
Modularity Opt. (t=0.7) & 0.85 & 0.72 & 0.26 \\
Spectral  Clustering & 0.86 & \textbf{0.80} & \textbf{0.38}\\
Normed Spectral Clust. & 0.84 & 0.77 & 0.25 \\
\bottomrule
\end{tabular}
\label{tab:mcc_im}
\end{table}

\begin{table}
\center
\caption{MCC, per database threshold}
\vspace{-0.5em}
\begin{tabular}{l c c c}
\toprule
 & Columbia & Carvalho & Korus \\
 \midrule
Splice Buster~\cite{cozzolino2015splicebuster} & 0.63 & 0.53 & 0.28 \\
Bondi et al.~\cite{bondi2017cvprw} & 0.45 & 0.29 & 0.14 \\
Huh et al. ``EXIF"~\cite{huh2018forensics}& 0.78 & 0.38 & 0.17 \\
\midrule
Modularity Opt. (t=0.7) & 0.80 & 0.65 & 0.19 \\
Spectral  Clustering & \textbf{0.82} & \textbf{0.75} & \textbf{0.31} \\
Normed Spectral Clust. & 0.79 & 0.70 & 0.20 \\
\bottomrule
\end{tabular}
\label{tab:mcc_db}
\end{table}

\begin{table}
\center
\caption{F1, per image threshold}
\vspace{-0.5em}
\begin{tabular}{l c c c}
\toprule
 & Columbia & Carvalho & Korus \\
 \midrule
Splice Buster~\cite{cozzolino2015splicebuster} & 0.78 & 0.62 & 0.36 \\
Bondi et al.~\cite{bondi2017cvprw} & 0.64 & 0.44 & 0.24 \\
%Huh et al. ``EXIF"~\cite{huh2018forensics}(reported) & 0.88 & 0.52 & \\
Huh et al. ``EXIF"~\cite{huh2018forensics}& \textbf{0.90} & 0.53 & 0.25 \\
\midrule
Modularity Opt. (t=0.7) & 0.88 & 0.73 & 0.26 \\
Spectral  Clustering. & 0.89 & \textbf{0.82} & \textbf{0.39} \\
Normed Spectral Clust. & 0.88 & 0.78 & 0.26 \\
\bottomrule
\end{tabular}
\label{tab:f1_im}
\end{table}

\begin{table}
\center
\caption{F1, per database threshold}
\vspace{-0.5em}
\begin{tabular}{l c c c}
\toprule
 & Columbia & Carvalho & Korus \\
 \midrule
Splice Buster~\cite{cozzolino2015splicebuster} & 0.74 & 0.59 & 0.30 \\
Bondi et al.~\cite{bondi2017cvprw} & 0.59 & 0.39 & 0.18 \\
Huh et al. ``EXIF"~\cite{huh2018forensics}& 0.82 & 0.45 & 0.20 \\
\midrule
Modularity Opt. (t=0.7) & 0.83 & 0.66 & 0.20 \\
Spectral Clustering & \textbf{0.86} & \textbf{0.77} & \textbf{0.32} \\
Normed Spectral Clust. & 0.83 & 0.70 & 0.20 \\
\bottomrule
\end{tabular}
\label{tab:f1_db}
\end{table}

\begin{table}
\center
\caption{Area Under the Curve (AUC)}
\vspace{-0.5em}
\begin{tabular}{l c c c}
\toprule
 & Columbia & Carvalho & Korus \\
 \midrule
Splice Buster~\cite{cozzolino2015splicebuster} & 0.79 & 0.68 & 0.56 \\
Bondi et al.~\cite{bondi2017cvprw} & 0.77 & 0.64 & 0.60 \\
Huh et al. ``EXIF"~\cite{huh2018forensics}& \textbf{0.96} & 0.72 & 0.57 \\
\midrule
Modularity Opt. (t=0.7) & 0.95 & 0.94 & \textbf{0.73} \\
Spectral  Clustering & 0.93 & 0.89 & 0.60 \\
Normed Spectral Clust. & 0.95 & \textbf{0.97} & 0.72 \\
\bottomrule
\end{tabular}
\label{tab:loc_auc}
\end{table}
